DOLOS: Tricking the Wi-Fi APs with Incorrect User Locations

Wi-Fi-based indoor localization has been extensively studied for context-aware services. As a result, the accurate Wi-Fi-based indoor localization introduces a great location privacy threat. However, the existing solutions for location privacy protection are hard to implement on current devices. They require extra hardware deployment in the environment or hardware modifications at the transmitter or receiver side. To this end, we propose DOLOS, a system that can protect the location privacy of the Wi-Fi user with a novel signal obfuscation approach. DOLOSis a software-only solution that can be deployed on existing protocol-compliant Wi-Fi user devices. We provide this obfuscation by invalidating a simple assumption made by most localization systems -- "direct path signal arrives earlier than all the reflections to distinguish this direct path prior to estimating the location". However, DOLOS creates a novel software fix that allows the user to transmit the signal wherein this direct path arrives later, creating ambiguity in the location estimates. Our experimental results demonstrate DOLOS can degrade the localization accuracy of state-of-art systems by 6x for a single AP and 2.5x for multiple AP scenarios, thereby protecting the Wi-Fi user's location privacy without compromising the Wi-Fi communication performance.

==> design/design-v7.tex <==
% !TEX root = paper.tex


\section{Threat Model}\label{sec:attack}
We formally describe the attack model and boil down to the requirements and the basic assumptions we make in designing \name's defense model.\looseness-1
{\color{red}ToDo: 1. discuss the situation of the enterprise network, the client's capability with multi-antenna, and AP's capability. 2. add 2.4ghz and 6ghz discussion for the sake of scope. 3. the scope of the threat model, e.g., if the attacker knows this defense 4. cots phone has linear array or not, which needs to be clarify. 5. seems that the reviewers need to know uplink/downlink obfus, and what knowledge we need to have for uplink obfuscation.}



\noindent \textbf{Attack scenario.} We consider the scenario in the Wi-Fi network (e.g., office buildings, malls, or other public venues), where a Wi-Fi AP is compromised or deliberately deployed by the attacker to communicate with the Wi-Fi users and reveal their location without their consent. We label this as the ``attacking'' AP. Since, we are considering a single AP localization system, one of the most reliable localization systems is to estimate the angle of arrival (AoA) and the time of flight (ToF) to the user to get the final user location. We seek to protect the billions of daily Wi-Fi users today whose location privacy is at stake. To provide this privacy protection, we explore how we can obfuscate the AoA and ToF measured by the attacking AP via a software-only solution.{\color{red}ToDo: add the discussion on when there is no reflection.}



\noindent \textbf{Attacking AP.} 
%Concerningly, both of these parameters can be determined without the user's consent, as this sensing can be a byproduct of the communication between the AP and the user. From a single received packet, 
The attacking AP can estimate AoA using numerous state of the art systems~\cite{spotfi, xie2018md, arraytrack, rapmusic,soltanaghaei2018multipath} from a single received packet. To estimate the ToF of the user from the attacking AP, WiPeep~\cite{wipeep} accurately measures the round trip time using the protocol-enforced ACK message generated by the user's Wi-Fi device. Through these systems, an attacking AP has two components to determine the user's location with decimeter-grade accuracy, and the user is rendered defenseless against the localization attack.  


\noindent \textbf{Wi-Fi user.} We consider the Wi-Fi users who can estimate the downlink wireless channel and leverage it to obfuscate his/her location through precoding the uplink data streams. 



\noindent \textbf{Scope.} To successfully deploy \name, we make two assumptions that often hold true in real-world settings:
\begin{itemize}[leftmargin=*] 
    \item The user device and the AP are equipped with multi-antenna, linear antenna arrays. 
    \item The wireless channel is reciprocal, i.e. the downlink (AP to user device) and uplink (user device to AP) channels are equivalent. 
\end{itemize}


\section{Primer on Wireless Localization}\label{sec:primer:localization}
The threat model provides the scope of the problem we are solving. In this section, we will first provide a quick primer on the necessary concepts needed to localize a user with a single AP. Second, we will also provide a naive solution that may work to obfuscate the user location but severely degrades the signal strength and communication throughput. 

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/primer-fig-crop.pdf}
    \caption{Wi-Fi-based localization with estimated AoA and ToF. After the Wi-Fi AP obtains the AoA $\theta_0$ and ToF $\tau_0$, the user's location is pinpointed. The right figure shows the profile with the SpotFi algorithm for AoA and ToF identification.}
    \label{fig:primer:localization}
\end{figure}



\subsection{Single AP Localization}%\label{sec:attack-model}


To localize the user in the Wi-Fi infrastructure, we consider the simple scenario where there are only direct path signals between the Wi-Fi AP and the user as shown in ~\cref{fig:primer:localization}. The Wi-Fi AP is trying to figure out the Wi-Fi user's coordinates (i.e., location) $\vec{p}_\mathrm{user}$ within his/her own coordinates $\vec{p}_\mathrm{AP}$. As a result, Wi-Fi AP can estimate the user's (x, y) coordinates by
$$ \vec{p}_\mathrm{user} = \vec{p}_\mathrm{AP} + c\tau_0*[\cos(\theta_0) \quad \sin(\theta_0)]^T, $$
where $\vec{p}_\mathrm{AP}$ is the location of the Wi-Fi AP, $\tau_0$ and $\theta_0$ are the estimated ToF and AoA in the AP's coordinates. Basically, AoA can tell in which direction the Wi-Fi user is and ToF can tell how far away the Wi-Fi user is. The Wi-Fi AP can run the SpotFi~\cite{spotfi} algorithm and further identify $\theta_0$ and the UbiLocate~\cite{pizarro2021accurate} algorithm to estimate the ToF $\tau_0$. Therefore, a single Wi-Fi AP can simply localize the Wi-Fi user with the above equation. The following illustrates how the attacker can obtain AoA and ToF for the Wi-Fi user's localization. 

\noindent \textbf{ToF estimation.} To estimate the distance between the attacker and the Wi-Fi user, we can estimate the round-trip time (i.e., $2\times$ToF) of the packets transmitted between the attacker and the Wi-Fi user. Then, the distance between the attacker and the Wi-Fi user is the multiplication of ToF and light speed. To do so, we can leverage the Fine Time Measurement (FTM) protocol~\cite{ftm_secure} to obtain the ToF of the packets transmitted between the attacker and the Wi-Fi user. To further tune the ToF estimation, we can leverage the wireless channel state information (CSI). As a signal travels over the air, it accrues additional phases depending on its frequency. A higher frequency signal will accrue a larger phase. We can leverage this fact to fine-tune the ToF measurements further. Specifically, a Wi-Fi signal is transmitted over multiple linearly spaced frequencies. Measuring the relative phase accumulation across these frequencies provides an estimate of the ToF of the signal. 

\noindent \textbf{AoA estimation.} After an attacking AP estimates the ToF, the attacker can figure out the distance between the attacker and the Wi-Fi user. To localize the Wi-Fi user, the attacker still needs to know in which direction the Wi-Fi user is. To this end, an attacking AP with multiple antennas can measure the phase difference of the incoming Wi-Fi signal between pairs of antennas to estimate the AoA. For simplicity, imagine two antennas spaced $d_\mathrm{sep}$ apart. The phase difference accrued between these two antennas is related to the AoA $\theta_0$ as 
$$\Delta \Phi = \exp(-\iota 2\pi \frac{1}{\lambda} d_\mathrm{sep} \sin(\theta_0)),$$ 
where $\lambda$ is the wavelength corresponding to the signal's center frequency and $d_{sep}$ is the antenna separation on the receiver. This additional phase difference is a consequence of the incremental distance signals travel to each of the receive antennas, as visualized in \cref{fig:intro}. Most of the existing localization algorithms rely on this fundamental effect to measure the AoA. 

These fundamental effects allow most localization algorithms to estimate the WiFi signal's path parameters. A visualization of the SpotFi transform, which estimates the ToF and AoA of the signal, is shown \cref{fig:primer:localization}. This profile will be used later as a visual aid to describe \name's obfuscation. 


\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/banner-channel-crop.pdf}
    \caption{\textbf{Wireless Channel based User Localization:} The user transmits a known precoded signal across $3$ time symbols from the $3$ antennas. The signals travel via multiple paths (green, blue) to the AP. The channel can be estimated based on the known transmitted signal. SpotFi~\cite{spotfi} is applied to segregate the paths across the angle and distance domain.}
    \label{fig:channel-model}
\end{figure*}

%\subsection{Path towards protecting privacy}\label{sec:attack-algo}
%To estimate the user's location, we need two measurements -- the time of flight and the angle of arrival. In WiPeep, the authors proposed a potential solution to protect against ToF measurements. However, their solution requires hardware changes and is only applicable to future Wi-Fi devices. 

\subsection{Nulling to the Direct Path} \label{sec:nulling}

To disable the attacking AP from leveraging the direct path signals for localization, a straightforward idea is to null the direct path. As a result, the attacking AP has to use multipath for localization, thereby, the location privacy is protected. To do so, we can create a nulling precoder $P_\mathrm{obf} = \vec{v_n}\vec{v_n}^H$, where $\vec{v_n}$ is the nulling vector in the direct path signal's null space, i.e. $\vec{v_d}^H \vec{v_n} = 0$. However, nulling the direct path will reduce the signal strength at the receiver and degrade the communication throughput at the attacking AP. Through experimental evaluation, we find the RSSI degrades by $6$ dB when the direct path is nulled. Instead, \name preserves all the paths and chooses to delay the direct path \textit{selectively} beyond the reflected paths to create ambiguity in AoA measurement. \name effectively increasing user localization error to over 3 meters while reducing signal strength by only $3$ dB. The impacts of nulling and \name's clever precoding are further characterized in \cref{sec:tput}. In the remaining sections, we will present how \name applies the appropriate precoding without affecting the channel capacity and obfuscates the channel unbeknownst to the attacking AP. 

 
\section{Designing Software-level Obfuscation}\label{sec:design}

We consider a single AP localization system to be one of the most deployable localization systems for Wi-Fi user localization. Most enterprise settings often deploy APs in an optimal fashion where only a single AP is visible to a Wi-Fi user. To comply with these realistic constraints, advancements have been made in AoA (Angle of Arrival) and ToF (Time of Flight) estimation to leverage these ubiquitous Wi-Fi signals for localization. 


\subsection{Intuition on location obfuscation}

In this section, we show how we can protect the Wi-Fi user's location privacy by obfuscating the wireless signals. Let's first compute the phases accrued at both the transmit and receive array of linearly spaced antennas due to the additional relative distance the signal travels:
\begin{equation}
    \vec{v_0}=\begin{bmatrix}
                1\\ 
                e^{-\iota2\pi d_\mathrm{sep}\sin\delta_0 / \lambda}\\ 
                e^{-\iota2\pi (2d_\mathrm{sep})\sin\delta_0 / \lambda}\\ 
                \vdots\\
                e^{-\iota2\pi (N_{TX}-1)d_\mathrm{sep}\sin\delta_0 / \lambda}
              \end{bmatrix} \, 
  \vec{u_0}=\begin{bmatrix}
                1\\ 
                e^{-\iota2\pi d_\mathrm{sep}\sin\theta_0 / \lambda}\\ 
                e^{-\iota2\pi (2d_\mathrm{sep})\sin\theta_0 / \lambda}\\ 
                \vdots\\
                e^{-\iota2\pi (N_{RX}-1)d_\mathrm{sep}\sin\theta_0 / \lambda}
              \end{bmatrix}
\end{equation}
If a transmitter steers power in the $\delta_0$ direction, the phases it must apply on its $N_{TX}$ antennas are given by $\vec{v}_0$. Similarly, if the receiver captures a signal coming from angle $\theta_0$, then the phases given in $\vec{u}_0$ will be accrued at the $N_{RX}$ antennas. These angles have been visualized in \cref{fig:channel-model}. For an $N_{RX} \times N_{TX}$ wireless system, the Wi-Fi signal's channel for a given single path, which is transmitted over $N_{sub}$ equally spaced frequency subcarriers, can be written as
$$ H_0(f_i) = a_0 \vec{u}_0 \vec{v}_0^H \exp(\iota 2\pi f_i \tau_0) \in \mathcal{C}^{N_{RX} \times N_{TX}},$$
where $a_0$ and $\tau_0$ are the direct path signal amplitude and ToF. As discussed in the introduction, we see the delays due to ToF appear as an additional phase dependent on the frequency of the $i^{th}$ subcarrier. 

However, the Wi-Fi signal reflections in the environment create ambiguities in AoA measurements. An example is shown in \cref{fig:channel-model}, with the direct path depicted by the green arrow and the reflection(s) by the blue arrow. If there are $M$ more paths that the signal takes to reach the receiver, the channel becomes

\begin{align}\label{eq:chan-ap}
    H(f_i)  = H_d(f_i) + \underbrace{\sum_{p=1}^M a_p \vec{u}_p \vec{v}_p^H \exp(\iota j 2 \pi f_i \tau_p)}_{\text{Reflections: } H_r}
\end{align}
where  $H_d(f_i)=a_d e^{-j 2 \pi f_i \tau_0} \vec{u}_d \vec{v}_d^H$ is the direct-path channel and $\vec{u}_d$ and $\vec{v}_d$ represent the steering vectors at the receiver and transmitter for direct path signals. Similarly, $\vec{u}_p$ and $\vec{v}_p$ represent the steering vectors at the receiver and transmitter for reflected path signals.


The reflections additively combine with the direct path channel defined previously and create ambiguous AoA measurements, $\theta_p$. 
However, the state-of-the-art localization algorithms assume the direct path, a straight line between the user and attacker AP, travels the least distance. The direct path is distinguished by either estimating the ToF through successive optimization~\cite{xie2018md, rapmusic} or via special transforms~\cite{spotfi, bloc, soltanaghaei2018multipath}, and choosing the path with the least ToF, $\tau_p$. An example of the Spotfi transform, which segregates the wireless channel according to the AoA and ToF is shown \cref{fig:channel-model}. Here, it is apparent that the direct path travels the least distance over the air and arrives first. The direct path's angle can be discerned from the y-axis. In \name, we seek to exploit this core assumption that the direct path always arrives the earliest to confuse the attacking AP. 


The following section will first discuss how the channel is estimated at the attacking AP (\cref{sec:chan-est}). In \cref{sec:design-bf}-\ref{sec:add-refs}, we build on the nulling idea explored previously to selectively delay only the direct path while preserving the communication throughput. 
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/banner-ablation-crop.pdf}
    \caption{(a) SpotFi profile of channel simulated assuming 4 RX antennas, 4 TX antennas, and 40 MHz bandwidth; (b) applying delay and beamforming towards direct path, both paths are delayed; (c) applying delay and beamforming \textit{solely} towards direct path and nulling elsewhere, removes reflections; (d) re-injecting reflections naively distorts the profile; (e) re-injecting reflections while aware of direct-path obfuscates channel.}
    \label{fig:precoding-ablation}
\end{figure*}

\subsection{Channel estimation at the attacking AP}\label{sec:chan-est}

In the standardized MIMO system, the wireless channel between each pair of transmitting and receiving antennas needs to be estimated as a necessary prerequisite to decoding the data. A known preamble sequence is used to estimate this channel. This sequence is transmitted across $N_{TX}$ symbols across all the transmit antenna, as shown in \cref{fig:channel-model}. The received signal for frequency $f_i$ across the $N_{RX}$ antennas and the $N_{TX}$ symbols is given by
\begin{align*}
    & R[f_i] = H(f_i) T[f_i], \quad H, R \in \mathcal{C}^{N_{RX} \times N_{TX}}, T \in \mathcal{C}^{N_{TX} \times N_{TX}} \\
    & \implies H(f_i) = R[f_i] T[f_i]^{-1}
    % & R[f_i] = H(f_i) T[f_i] \implies H(f_i) = R[f_i] T[f_i]^{-1} \\
    % & where \quad H(f_i) \in \mathcal{C}^{N_{TX} \times N_{RX}}, and \quad R[f_i], T[f_i] \in \mathcal{C}^{N_{TX} \times N_{TX}} \\
\end{align*}

To ensure the channel can be reliably estimated, an invertible $T$ is chosen. It is simply constructed across all frequencies by considering a preamble symbol $\vec{L} \in \mathcal{C}^{N_{sub}}$, and an invertible precoding matrix $P[f_i] \in \mathcal{C}^{N_{TX} \times N_{TX}}$. Hence, the user can transmit the data $T[f_i] = P[f_i] \vec{L}[i]$ that is precoded by the precoding matrix, and the channel is estimated via 
$$H(f_i) = \frac{R[f_i]}{\vec{L}[i]} P[f_i]^{-1}$$ 
which will be used by the attacker to localize the user. As a result, the user can manipulate the precoding matrix of  $P[f_i]$ to obfuscate his/her location. 


Since the channel is estimated at the receiver, a user does not have any impact on the way the attacker measures the channel or how it traverses the environment. Hence, many past works~\cite{yao2018aegis, staat2022irshield} seeking to obfuscate user locations deploy additional hardware in the environment to change the wireless channel explicitly, making their widescale implementation challenging. However, the user does have control over the precoding ($P[f_i]$) they can apply on the preamble sequence at a software level. Hence, without loss of generality, if the attacking AP expects an identity matrix to be applied as precoding, but the user instead applies a precoding matrix $P_\mathrm{obf}[f_i]$, the attacking AP will measure an incorrect obfuscated channel 
\begin{align}
    H(f_i)_\mathrm{obf} &= H(f_i) P_\mathrm{obf}[f_i] \nonumber \\
                        &= a_d e^{-j 2 \pi f_i \tau_0} \vec{u}_d \vec{v}_d^H P_\mathrm{obf}[f_i] + H_r(f_i) P_\mathrm{obf}[f_i] \label{eq:chan_obf} 
\end{align}
Next, we will illustrate how we can manipulate the precoding matrix such that the user's location is obfuscated and the communication throughput is maintained. 

% \begin{table}[]
%     \small
%     \begin{tabular}{|c|c|c|cccc|}
%     \hline
%     \multirow{2}{*}{} &
%       \multirow{2}{*}{No obf.} &
%       \multirow{2}{*}{Null} &
%       \multicolumn{4}{c|}{Preserve paths and delay } \\ \cline{4-7} 
%      &  &  & \multicolumn{1}{c|}{0 (m)} & \multicolumn{1}{c|}{20 (m)} & \multicolumn{1}{c|}{30 (m)} & 40 (m) \\ \hline
%     AoA error &
%       $0^\circ$ &
%       $62^\circ$ &
%       \multicolumn{1}{c|}{$0^\circ$} &
%       \multicolumn{1}{c|}{$58^\circ$} &
%       \multicolumn{1}{c|}{$61^\circ$} &
%       $53^\circ$ \\ \hline
%     \begin{tabular}[c]{@{}c@{}}RSSI\\ (dBm)\end{tabular} &
%       -65 &
%       -71 &
%       \multicolumn{1}{c|}{-64} &
%       \multicolumn{1}{c|}{-64} &
%       \multicolumn{1}{c|}{-64} &
%       -62 \\ \hline
%     \end{tabular}
%     \caption{Received signal strength for different obfuscation techniques}
%     \label{table:aoa_rssi}
% \end{table}


\subsection{Selective beamforming and controlled delay}\label{sec:design-bf}



{\color{red} ToDo: 1. add a description of the symbols before using it. 2. channel estimation process should be more detailed 3. put some results (e.g., throughput is not compromised without design) here to make the flow smooth and understandable}
\name's core deliverable is to increase $\tau_0$, the direct path's time of flight, to a number larger than that of the reflections. It should achieve this by minimally impacting the rest of the channel. The simplest way to achieve this is to beamform solely in the direction of the direct path, and apply the necessary delay to the channel. In this case, $P_\mathrm{obf} = \vec{v_d}\vec{v_d}^H \exp(j 2\pi f_i \tau_\mathrm{delay})$. This effectively delays the direct path but at the detrimental cost of delaying the multipath signals by similar amounts. This is visually depicted for an example beamforming pattern in \cref{fig:ant-pattern}. It is clear that the direct path beamformer (orange), leaks power in the direction of the reflections (pink). This can lead to the reflections accruing the same delays as the direct paths. Hence leaving the relative ToFs between the various paths unchanged and allowing the attacking AP to discern the direct path as the earliest arriving signal. The impact of this is shown in \cref{fig:precoding-ablation}(b), wherein both the direct path and reflected paths are delayed by similar amounts when compared to the original channel in \cref{fig:precoding-ablation}(a). Hence, our first insight is to apply delay via an appropriate precoder without impacting the reflections in $H_r$.

A simple and effective precoder hence lies in the null space of $H_r$, which ensures power is not directed in the directions of the reflections. Since $H_r$ is the channel devoid of direct path, it is not full rank, implying the existence of at least one such null vector $\vec{n}_r$. We can then construct $P_\mathrm{obf} = \vec{n}_r \vec{v}_d^H \exp(j 2\pi f_i \tau_\mathrm{delay})$. This is shown by the blue beamformer in \cref{fig:ant-pattern}. This beamformer does not direct power in the direction of the reflection, allowing \name to solely delay the direct path. However, the nulling vector does not align with the direct path direction perfectly, and can create incorrect delays applied to the channel. Specifically, we have $\vec{v}_d^H\vec{n}_r = \alpha \exp(j\phi)$ which needs to be explicitly compensated for within the precoder, giving us
$$P_\mathrm{obf}[f_i] = \frac{1}{\alpha}\vec{n}_r \vec{v}_d^H \exp(j 2\pi f_i \tau_\mathrm{delay} - \phi)$$
As a result, the direct-path channel will be properly delayed without affecting the reflected paths.

\todo{cite mimo paper, talking about spatial multiplexing}

Unfortunately, this precoder, which lies in the null space of the reflected paths, entirely suppresses these reflections which are crucial to obfuscate the channel, i.e., $H_r (f_i) P_\mathrm{obf}[f_i] = 0$. This additionally reduces the channel capacity by reducing the spatial multiplexing gain, the ability to support multiple parallel streams of data communication, which negatively affects the overall throughput of the MIMO system leading to lower data rates. This impact is visualized in \cref{fig:precoding-ablation}(c).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/bf-nulling-antenna-pattern-crop.pdf}
    \caption{Antenna patterns show power directed towards different directions. Without nulling, power is directed towards direct path and reflections, delaying both paths equally}
    \label{fig:ant-pattern}
\end{figure}




\subsection{Adding back the reflections} \label{sec:add-refs}
{\color{red} ToDo: 1. clearly specify the distortion introduced by adding hr 2. distinction between the authorized access network and attacker. are they the same? why attacker cannot get encryption key?}

We can supplement the precoder with a beamformer directing power along the reflected paths to bring these reflections back. However, naively adding back $H_r$ creates distortions to the channel as visualized in \cref{fig:precoding-ablation}(d). This is a consequence of non-zero power directed in the direction of the direct path.  
Clearly, adding back the reflections is trickier than it seems at first glance, as any changes we now make to the precoding impact the direct path delays as well. 

We can circumvent the impact on the direct path by simply choosing to reconstruct the multipath components using the null vectors of the direct path steering vector $v_d$. Specifically, given the null space of $\vec{v}_d^H$ as $N \in \mathcal{C}^{N_{TX} \times (N_{TX}-1)}$, the goal is to supplement the above precoder with an additional component which is closest to identity, 
\begin{align*}
    P_\mathrm{supplement}[f_i] = NA \approx I \implies A = N^H (N N^H)^{-1} 
\end{align*}
This supplementary precoder will not impact the direct path component of the channel but will reintroduce the multipath most effectively. Hence, \name's final precoder is
\begin{align}
P_\mathrm{obf}[f_i] = \frac{1}{\alpha}\vec{n}_r \vec{v}_d^H \exp(j 2\pi f_i \tau_\mathrm{delay} - \phi) + N N^H (N N^H)^{-1} \label{eq:prec-bf-delay}
\end{align}
In this way, even though we add back the reflections, the direct path signals will not be affected. The impact of applying this precoder on our channel is shown in \cref{fig:precoding-ablation}(e).

\section{Real-world Considerations}

The previous section discussed the precoding \name applies to obfuscate the channel. This precoding selectively delays the signal transmission along the direct path to ensure that the first signal arriving at the attacking AP is a reflection. This creates ambiguity for the attacker in estimating the direct path's AoA and ToF, hence obfuscating the user's location. However, there are a few real-world considerations before implementing the system. This section will delve into these considerations. First, we will explore how the direct path and reflections' parameters were estimated in \cref{sec:design}. Next, we will discuss how this precoding can be reversed by legitimate AP's providing location services to the user. Finally, we will strengthen the obfuscation to an attacker who is trying to circumvent \name.  

\subsection{Estimating path parameters}\label{sec:est-path-params}

\todo{goes to implementation}
With the precoder mathematically defined, we need to estimate the core variables that are key to creating this precoder on the user's device. To compute the precoding, we need knowledge of the uplink channel, the wireless channel when the user transmits to the AP, collected at the attacking AP. We can rely on channel feedback, wherein the AP informs the user of the uplink channel and is a standard part of MIMO communication. However, if the attacking AP has access to an unobfuscated channel, it defeats our efforts. Instead, we assume that the channel is reciprocal, and note that before connecting to an AP, the user's Wi-Fi device will listen to the AP-discovery packet. The hermitian of the downlink channel measured on this packet can be assumed to be the uplink channel we need~\cite{tse2005fundamentals}. 

We can now compute the precoding with access to the pseudo-uplink channel. The two components of the precoder require the direct path channel and the channel comprising the reflections. We have to tease apart that direct path and reflected path components. We can reliably do this via mD-Track~\cite{xie2018md}. However, due to noise in channel measurements, we average the channel across 20 beacon packets~\cite{arraytrack}, before estimating the path parameters and connecting to a Wi-Fi access point. 

\subsection{Precoding Matrix as an Encryption Key} \label{sec:reverse-obf}

While we can see that using \name would obfuscate the user location with the attacking access point, we also want to ensure that an authorized access network can still locate the user. To that end, in \name we propose to use the precoding matrix estimated in \cref{eq:prec-bf-delay} as the encryption key that could be sent over to the authorized access network, to decrypt the user location as needed. Revisiting \cref{eq:chan_obf}, the true channel, and subsequently the true AoA, can be estimated by taking an approximate inverse of the precoding matrix ($P_\mathrm{obf}^\dagger$) that has been provided by the user, 
\begin{align*}
    H(f_i)_\mathrm{obf} P_\mathrm{obf}^\dagger[f_i] = H(f_i)P_\mathrm{obf}[f_i]P_\mathrm{obf}^\dagger[f_i] \approx H(f_i)
\end{align*}

This inverse precoding matrix, $P_\mathrm{obf}^\dagger$, can be sent over the air while applying cryptographically secure encryption. 

\subsection{Obfuscating despite knowing defense}\label{sec:mirage-known}
{\color{red}ToDo: need more details and security analysis rigorously. I think we should either put it at the discussion or do micro-benchmark or simulation here.}
A clever attacker may try to circumvent the defenses provided with this system. A simple way to circumvent this attack is by averaging packets across multiple time steps. As the user moves through space, often the angle of arrival of reflections in the environment changes more rapidly as opposed to the direct path links. The direct path is hence more stable across these packets. If the attacker collects Wi-Fi packets over several seconds and averages the channel over these packets, they can effectively reduce the impact of reflections in the environment while strengthening the effects of the direct path. This is often done in Wi-Fi localization systems~\cite{arraytrack} to further improve localization accuracy. By reducing the effects of reflections in the perceived channel, \name cannot ``hide'' the direct path amongst reflections, impairing our obfuscation capabilities. A simple insight can protect against this attack -- impart a similar randomness to the direct path as well. We can do this by effectively applying random delays, $\tau_\mathrm{delay}$ to the direct path. This will ensure the direct path representation is also weakened during the averaging operation, affecting the attackers ability to measure the direct path's AoA and ToF. 



==> intro/intro-v10.tex <==
\section{Introduction}

% Para 1 -- Wi-Fi based localization has been recongozed and imprtatn for decimeter accurate lcoation.
% The research started at a few meters accurate to now being decimeter acccurate.
User's location in indoor scenarios is an important aspect of providing a personalized experience.
It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automation~\cite{arun2022p2slam}.
For these applications and many more, localization accuracy on the order of tens of centimeters is key.
This led to accurate Wi-Fi based indoor localization research for more than two decades that started with signal strength (RSSI) localization systems that can provide only a meter-accurate localization~\cite{radar,zee} to many recent systems~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} that provide tens of centimeters-accurate user location using Wi-Fi signal's physical-layer information. 

% Para 2 -- Rssi based meter level accurate systems have been improved by the current works achieve decimeter accurate by doing aoa, tof and do not require consent, hence privacy concerns.
Wi-Fi based localization algorithms primarily rely on three measurements to determine a user's location in these scenarios - the received signal strength (RSSI), the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. 
Concerningly, many of these systems can operate without the consent of the user due to two main reasons: (i) These measurements for a user devices transmission happen at the WI-Fi AP, and (ii) A mixture of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA measurements can be successfully used to localize a user to decimeter-level accuracy and invade their location privacy.


On the other hand, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar, ez}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. 
So, in this paper we aim to deteriorate current AoA and ToF based localization systems' accuracies form decimeter-accurate to meter-accurate (or as bad as RSSI based localization systems). Further, a perfect defense should not need any additional hardware or firmware changes, and also not disrupt the user's internet connectivity through the Wi-Fi network.
% In contrast, a mixture of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA measurements can be successfully used to localize a user to decimeter-level accuracy and invade their location privacy. So, ideally, we would like to disable AoA and ToF-based localization algorithm's accuracy to deteriorate 10s of centimeter median error localization systems to be erroneous to a few meters or as inaccurate as an RSSI-based system.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/intro-fig-ieee-sp-crop.pdf}
    \caption{(a) \name-disabled Wi-Fi user can be accurately localized by the Wi-Fi APs thereby introducing the location privacy threat. (b) \name-enabled Wi-Fi user can obfuscate the wireless signals for location privacy protection.}
    \label{fig:main-intro-fig}
\end{figure}

% Para 3 -- Some works for privacy falls short of doing a good job.
% There are a few works that defend against these attacks by masking the user identifity by anonymizing the MAC address with which the user connects to the Wi-Fi network~\cite{zhong2004privacy,alaggan2018privacy}. However, recent works~\cite{givehchian2023practical} have shown that chip-level imperfections cause distortions in the signals that can be used to fingerprint devices and identify users despite MAC randomization. 
Current ToF based localization systems try to ensure that user can alone make their measurements, and the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{802.11az} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} demonstrates an attack on 802.11mc FTM, that would still translate to the current state-of-the-art wireless sensing systems.
% An alternative to masking user identity is to disrupt the localization measurements.
% WiPeep~\cite{wipeep} also proposes a solution to their demonstrated vulnerability in FTM measurements. However, the proposed solution requires changing packet transmission times and is only applicable to future wireless devices, {\todo{this is hard to understand to me: and thus if desired a given access point can determine the ToF to a user device. }}
On the other hand, a few works have explored disabling an AP's ability to localize altogether, by deploying a repeater~\cite{yao2018aegis} or Smart surface~\cite{staat2022irshield} in the environment, tuning the signal's phase and amplitude to prevent a receiver from localizing the user. 
Although these systems prevent the Angle of Arrival (AoA) determination, they require additional hardware to be deployed in the environments and do not provide a scalable solution for all spaces. 
% So, it is important that the privacy system to not need any hardware or {\todo{ our method needs firmware change?: firmware changes}} that can be deployed on current user devices. {\todo{we can mention these extra smart surfaces and repeaters are compromising the wireless communications as well}}

% Para 4 --We do a good job by making the decimeter systems as inaccurate as rssi-systems or accurate to only a few meters. Our system is also protocol-compliant and communication preserving. So let us understand what makes this challenging.
So, we design \name, a system to protect users from being localized without consent in the public or enterprise networks. \name's defense is against the attacker that either could compromise one or more access points (APs), within the public or enterprise networks.
\name's defense model is to deteriorate the AoA and ToF-based localization accuracy of the Wi-Fi localization algorithms to be as inaccurate as RSSI-based localization, i.e., an average of 2-3m median accurate location estimation.
Additionally, \name makes use of the existing precoding protocols in Wi-Fi~\cite{beam_forming_doc} to precode the signal prior to transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. 
This allows \name to readily integrate into most existing Wi-Fi devices and provide user-location privacy with only a software fix.
Finally, to ensure user's location privacy without compromising their connectivity to the Internet, we design \name to have no disruption to the existing communication link


% Para 5 -- First challenge is that the APs have multiple antennas that can resolve multiple paths through aoa estimation, and identify the direct path using the notion that it is the least travelled and most consistent path.
The first design challenge \name attempts to resolve is that, while carrier frequency-based phase-shifts can achieve decent ToF unreliability~\cite{olafsdottir2017security,riaz2022security,staat2022analog}, APs designed for MIMO communication have multiple antennas that can overcome them by performing AoA measurements. As shown in Figure~\ref{fig:main-intro-fig}(a), state-of-the-art Single-AP based decimeter-accurate localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az} rely on a simple fact when they use channel state information (CSI) to estimate accurate ToF and AoA -- "direct-path travels the least amount of time in the air". This helps the algorithms to distinguish the direct path parameters from the reflected path's parameters to estimate accurate ToF~\cite{802.11az} and accurate AoA~\cite{spotfi}.
So, \name's first key idea is to obfuscate the direct path such that the first of the reflected paths appears to be the shortest traveled path. This would in turn lead to inaccurate AoA and ToF estimates, degrading their localization accuracy to be of the order of a few meters as shown in Figure~\ref{fig:main-intro-fig}(b).

% Para 6 -- A dumb way to do this is nulling but reduces the communication link, so we firstly precode such that the ap does not perceive the correct direct path and also does not remove any paths thus maintatining communication link.
A simple way to make the algorithm estimate the reflected path to be the shortest path is to simply remove the direct path as shown in Figure~\ref{fig:intro}(b). Unfortunately, this removes one of the dominant paths for connectivity, reducing the throughput of the user connection. Thus we cannot simply remove the direct path signal. Another key observation we note here is that, for a given location of the user and the Wi-Fi AP, we cannot change the directions or AoAs of the received signal as that depends on the geometry of the environment that is out of our control or would need additional hardware deployments that compromise deployability of \name's design. So, in \name we identify that the only way we can let the receiver perceive the reflected path to be the shortest traveled path is if we can "delay" the signal along the direct-path direction.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-usenix-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to AoA across receive antennas}
    \label{fig:intro}
\end{figure}
% Para 7 -- The second challenge, is that delaying one-path creates delays or ghost peaks across all the paths like done in mirage, so we need to ensure that the direct path and multipath precoding matrices are orthogonal and that we add delay to only the direct path's precoding vector.
Since the multiple reflections (multipath) in the environment, including the direct path and the reflected paths, have a common source, a naive beamforming as performed by the authors in MIRAGE~\cite{ayyalasomayajula2023users} that applies a delay to the transmitted signal, unfortunately, would delay all the signals in all directions by the same amount as shown in Figure~\ref{fig:intro}(c). Here \name makes a key observation that most of the modern user device relies on MIMO communication and thus have multiple antennas for transmission. This would imply that the user device can beamform~\cite{beam_forming_doc} the signal independently in each of the signal departure directions or angle-of-departures (AoD). Thus, in \name we design an optimized precoding matrix that is conditioned to beamform the transmitted signal while ensuring that both:
(a) The beamforming along the direct path with additional delay is orthogonal to the reflected path's transmitted directions.
(b) The beamforming performed for the reflected paths without additional delays is orthogonal to {\todo{ we ensure there is not interference between direct and reflected paths, thereby orthogonal to the direct path?: the newly delayed reflected path's transmitted directions.}}

% Para 8 -- Finally, we address a few real world problems of consistency of the direct path and multiple collaborative APs, by adding random delays and obfuscating one AP at a time across all the environment AP respectively.
Finally, \name also addresses two key real-world problems to make the system robust to a range of attacks: (a) Since, direct-path is always more consistent {\todo{ I don't understand here: than overtime than reflected path~\cite{spotfi},}} an attacker who has knowledge of \name can simply cluster packets across time as done in ~\cite{spotfi} to get the most consistent path. We ensure to overcome this by randomizing the obfuscation delay added to the direct path, so even the direct path is {\todo{no longer?}}longer consistent over time. (b) An attacker can also compromise multiple APs~\footnote{With the exception of all the APs in monitor mode which would greatly reduce the communication capacity of the environment, {\todo{ which is against the original purpose of Wi-Fi infrastructure deployment.}}}, to locate the user. {\todo{seems the sentence is broken. do we need to mention this?: So, in \name we ensure that we demonstrate how the measurements can previous timesteps can still be used for current transmissions obfuscation with the observation that compared to the communication link rate, the user motion is more quasi-static. }}


\name's obfuscation is tested on commercially available Wi-Fi radios~\cite{warp}, across 30 locations and over 1000 packets in realistic settings. \name's design degrades the accuracy for fundamental predictions of AoA and ToF that are used by the state-of-the-art localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az}. So we compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} (relies fundamentally on AoA) and UbiLocate~\cite{pizarro2021accurate} (relies fundamentally on ToF). Through these experiments, we demonstrate the efficiency of \name on Wi-Fi user's location protection. Our experimental results show the localization error degrades by $\sim6\times$ at the median with localization errors as high as $1.33$ m in a $4$m$\times4$m space, AoA estimation error degrades by $20\times$ at the median, and ToF estimation error degrades by $\sim2.5\times$ at the median after \name. 


{\todo{we need the contribution section}}

==> intro/intro-v12.tex <==
\section{Introduction}

% Para 1 -- Wi-Fi based localization has been recongozed and imprtatn for decimeter accurate lcoation.
% The research started at a few meters accurate to now being decimeter acccurate.
User's location in indoor scenarios is an important aspect of providing a personalized experience.
It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automation~\cite{arun2022p2slam}.
For these applications and many more, localization accuracy on the order of tens of centimeters is key.
This led to accurate Wi-Fi-based indoor localization research for more than two decades that started with signal strength (RSSI) localization systems that can provide only a meter-accurate localization~\cite{radar,zee} to many recent systems~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} that provide tens of centimeters-accurate user location using Wi-Fi signal's physical-layer information. 

% Para 2 -- Rssi based meter level accurate systems have been improved by the current works achieve decimeter accurate by doing aoa, tof and do not require consent, hence privacy concerns.
Wi-Fi-based localization algorithms primarily rely on three measurements to determine a user's location in these scenarios - the received signal strength (RSSI), the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. 
Concerningly, many of these systems can operate without the consent of the user due to two main reasons: (i) These measurements for a user device transmission happen at the WI-Fi AP, and (ii) A mixture of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA measurements can be successfully used to localize a user to decimeter-level accuracy and invade their location privacy.


On the other hand, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar, ez}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. 
So, in this paper, we aim to deteriorate current AoA and ToF-based localization systems' accuracy from decimeter-accurate to meter-accurate (or as bad as RSSI-based localization systems). Further, a perfect defense should not need any additional hardware or firmware changes and also not disrupt the user's internet connectivity through the Wi-Fi network.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/intro-fig-ieee-sp-crop.pdf}
    \caption{(a) \name-disabled Wi-Fi user can be accurately localized by the Wi-Fi APs, thereby introducing the location privacy threat. (b) \name-enabled Wi-Fi user can obfuscate the wireless signals for location privacy protection.}
    \label{fig:main-intro-fig}
\end{figure}

% Para 3 -- Some works for privacy falls short of doing a good job.
Current ToF-based localization systems try to ensure that user can alone make their measurements, and the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{802.11az} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} demonstrates an attack on 802.11mc FTM, that would still translate to the current state-of-the-art wireless sensing systems.
On the other hand, a few works have explored disabling an AP's ability to localize altogether by deploying a repeater~\cite{yao2018aegis} or Smart surface~\cite{staat2022irshield} in the environment, tuning the signal's phase and amplitude to prevent a receiver from localizing the user. 
Although these systems prevent the Angle of Arrival (AoA) determination, they require additional hardware to be deployed and do not provide a scalable solution for all spaces. 

% Para 4 --We do a good job by making the decimeter systems as inaccurate as rssi-systems or accurate to only a few meters. Our system is also protocol-compliant and communication preserving. So let us understand what makes this challenging.
We design \name, a system to protect users from being localized without consent in the public or enterprise networks. \name's defense is against the attacker that could compromise one or more access points (APs), within the public or enterprise networks.
\name's defense model is to deteriorate the AoA and ToF-based localization accuracy of the Wi-Fi localization algorithms to be as inaccurate as RSSI-based localization, i.e., an average of 2-3m median accurate location estimation.
Additionally, \name's design uses existing precoding protocols in Wi-Fi~\cite{beam_forming_doc} to precode the signal before transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. 
This allows \name to readily integrate into most existing Wi-Fi devices and provide user-location privacy with only a software fix.
Finally, to ensure user's location privacy without compromising their connectivity to the Internet, we designed \name to have no disruption to the existing communication link.


% Para 5 -- First challenge is that the APs have multiple antennas that can resolve multiple paths through aoa estimation, and identify the direct path using the notion that it is the least travelled and most consistent path.
The first design challenge \name attempts to resolve is that, while carrier frequency-based phase-shifts can achieve decent ToF unreliability~\cite{olafsdottir2017security,riaz2022security,staat2022analog}, APs designed for MIMO communication have multiple antennas that can overcome them by performing AoA measurements. As shown in Figure~\ref{fig:main-intro-fig}(a), most localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az} rely on a simple fact when they use channel state information (CSI) to estimate accurate ToF and AoA -- ``direct-path, as compared to the reflections, travels the least amount of time in the air''. Filtering the signals across the time domain helps these systems to reduce the impact of reflections in the environment, a significant source of error, and estimate accurate ToF~\cite{802.11az} and AoA~\cite{spotfi} to furnish decimeter-level accuracy.
So, \name's first key idea is to obfuscate the direct path such that the first of the reflected paths appears to be the shortest traveled path. This would, in turn, lead to inaccurate AoA and ToF estimates, degrading their localization accuracy to be of the order of a few meters as shown in Figure~\ref{fig:main-intro-fig}(b).

% Para 6 -- A dumb way to do this is nulling but reduces the communication link, so we firstly precode such that the ap does not perceive the correct direct path and also does not remove any paths thus maintatining communication link.
A simple way to make the algorithm estimate the reflected path as the shortest path is to remove the direct path, as shown in Figure~\ref{fig:intro}(b). This removes one of the dominant paths for connectivity, reducing the throughput of the user connection. Thus, we cannot simply remove the direct path signal. We also note that for a given location of the user and the Wi-Fi AP, we cannot change the directions or AoAs of the received signal as that depends on the geometry of the environment that is out of our control or would need additional hardware deployments that compromise deployability of \name's design. So, in \name we identify that the only way to let the receiver perceive the reflected path as the shortest traveled path is to ``delay'' the signal along the direct-path direction.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-usenix-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to AoA across receive antennas}
    \label{fig:intro}
\end{figure}
% Para 7 -- The second challenge, is that delaying one-path creates delays or ghost peaks across all the paths like done in mirage, so we need to ensure that the direct path and multipath precoding matrices are orthogonal and that we add delay to only the direct path's precoding vector.
Since the multiple reflections (multipath) in the environment, including the direct path and the reflected paths, have a common source, naive beamforming as performed by the authors in MIRAGE~\cite{ayyalasomayajula2023users} that applies a delay to the transmitted signal, unfortunately, would delay all the signals in all directions by the same amount as shown in Figure~\ref{fig:intro}(c). Here, \name makes a key observation that most modern user devices rely on MIMO communication and thus have multiple antennas for transmission. This would imply that the user device can beamform~\cite{beam_forming_doc} the signal independently in each of the signal departure directions. Thus, in \name we design an optimized precoding matrix that is conditioned to beamform the transmitted signal while ensuring that both:
(a) The beamforming along the direct path with additional delay is orthogonal to the reflected path's transmitted directions.
(b) The beamforming performed for the reflected paths \textit{without} additional delays is orthogonal to the newly delayed reflected path's transmitted directions.

% Para 8 -- Finally, we address a few real world problems of consistency of the direct path and multiple collaborative APs, by adding random delays and obfuscating one AP at a time across all the environment AP respectively.
Finally, \name also addresses a key real-world problem to make the system robust to a potential way to circumvent \name's obfuscation. Since direct path is always more consistent across time than reflected path~\cite{spotfi}, an attacker who has knowledge of \name can cluster packets across time as done in ~\cite{spotfi} to get the most consistent path. However, we can protect against this by randomizing the obfuscation delay added to the direct path and creating artificial inconsistencies in the perception of the direct path.  
% (b) An attacker can also compromise multiple APs, to locate the user. We demonstrate \name such that it can obfuscate each AP the user is connected to.


We bring these ideas together, and \name's obfuscation is tested on commercially available Wi-Fi radios~\cite{warp} across 30 locations and over 1000 packets in realistic settings. \name's design degrades the accuracy for fundamental predictions of AoA and ToF that are used by the state-of-the-art localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az}. So we compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} (relies fundamentally on AoA) and UbiLocate~\cite{pizarro2021accurate} (relies fundamentally on ToF). Through these experiments, we demonstrate the efficiency of \name on Wi-Fi user's location protection. Our experimental results show the localization error degrades by $\sim6\times$ at the median with localization errors as high as $1.33$ m in a $4$m$\times4$m space, AoA estimation error degrades by $20\times$ at the median, and ToF estimation error degrades by $\sim2.5\times$ at the median after \name. 

\noindent\textbf{Our Contributions:}
\begin{itemize}[leftmargin=*]
    \item \name's defense obfuscates all of the current decimeter accurate localization systems by up to $6\times$, and ensures at best a meter-level or worse accuracy.
    \item \name's defense does not require any hardware or firmware changes, and is Wi-Fi standard compliant.
    \item An attacker cannot counter \name despite of their knowledge of \name's implementation, owing to the randomization of obfuscation delay.
\end{itemize}

% {\todo{we need the contribution section}}

==> intro/intro-v6.tex <==
% how to locate --> preserve privacy by attacking these ways --> but not broadly applicable --> create software-only by digitally chaging transmission phases --> 
\section{Introduction}

User's location in indoor scenarios is an important aspect of providing a personalized experience. It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automations~\cite{arun2022p2slam}. For these applications and many more, localization accuracy on the order of tens of centimeters is key. Given the widespread presence of WiFi networks indoors, many works~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} have developed systems to provide user location using WiFi signal's physical-layer information. Concerningly, however, many of these systems can operate without the consent of the user. A user connected to just a single access point in an environment can be localized within the required accuracy via the exchange of just a few wireless communication packets~\cite{vasisht2016decimeter}. This compromises user location privacy and opens the door for organizations to potentially commodify~\cite{origin_wireless} to even deploy in homes~\cite{lee2016smart} and spy on users in public spaces~\cite{zhu2018tu}. This underscores the urgency of safeguarding location privacy from potential intrusions by these localization systems.   


\name develops a method to protect users of public or enterprise networks from being localized indoors without consent. In realistic WiFi networks, access points are deployed optimally such that only a single AP provides coverage in most locations. This provides a cost-effective deployment in large indoor spaces and reduces interference from neighboring access points, improving signal integrity. Consequently, user devices only connect and communicate with a single AP at a time. Single-AP localization solutions have hence been deployed~\cite{vasisht2016decimeter} to tackle these scenarios. Three measurements are primarily used to determine a user's location in these scenarios - the signal strength, the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. However, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. A combination of ToF (802.11mc) and AoA can instead be successfully used to localize a user to decimeter-level accuracy and invade their location privacy. 

The first line of defense against these intrusive attacks is to anonymize the MAC address with which the user connects to the WiFi network. This masks the user's true identity from the network, and although they can be localized, they cannot be identified. However, recent works~\cite{givehchian2023practical} have shown that chip-level imperfections cause distortions in the signals that can be used to fingerprint devices, and identify users despite MAC randomization. Alternative to masking the user's identity, few works have explored disabling an AP's ability to localize altogether. WiPeep~\cite{wipeep} proposed a solution to the vulnerability in FTM measurements, which allowed APs to measure FTM outside of a protocol-compliant ranging session. However, their solution requires changing packet transmission times, which need to be implemented via hardware/firmware changes and is only applicable to future wireless devices. Instead, Aegis~\cite{yao2018aegis} deploys a repeater in the environment which tunes the phase and amplitude of a signal to prevent a receiver from localization. IRSheild~\cite{staat2022irshield} implements a similar technique, but with the use of an Intelligent Reflective Surface to inject phase noise in the WiFi measurements. 
Finally, the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{au2022guest} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} would still translate.
Although these systems prevent the AoA determination, they require additional hardware to be deployed and do not provide a scalable solution for all environments. Instead, \name precodes the signal prior to transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. This approach can be integrated into most existing WiFi devices without the need for additional hardware or firmware changes with minimal disruption to the communication link.

% ----
As discussed, AoA forms a core part of estimating the location of the user with decimeter-level accuracy. Most multi-antenna access points have the ability to measure AoA by observing the relative phase accrued between pairs of their antennas. This relative phase is accrued as the signal travels a slightly larger distance to some antennas than others, as shown in the central inset in \cref{fig:intro}. Clearly, this physical effect is a consequence of how the signal propagates through the environment and remains consistent regardless of the transmission. Consequently, prior works primarily seek to make changes to the environment by deploying specialized hardware. Does this then preclude a software-only obfuscation scheme? Not necessarily. The measurement of AoA is complicated by the presence of signal reflection(s) in the environment, as shown by the blue arrows in \cref{fig:intro}. Our first insight is to leverage these reflections to create ambiguity in the attacker's AoA estimation by applying a specialized precoding scheme.  


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-sigcomm-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays only the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to non-zero angle of arrival across receive antennas}
    \label{fig:intro}
\end{figure}


To enable localization despite reflections, an AP needs to measure the AoA of the direct path signal arriving from the user device. To distinguish these direct path signals from reflections, existing single-AP solutions~\cite{singleap, chronos, soltanaghaei2018multipath} rely on a core assumption -- the direct path signal travels the least distance and arrives earlier \footnote{delayed by an order of tens of nanoseconds} than the other paths. So, a simple way to provide obfuscation is for a user device to transmit purely in the direction of the reflections, i.e. introduce a null in the direction of the direct path and remove the direct path from the picture as shown in \cref{fig:intro}(b). Despite its effectiveness, this nulling will drastically impact the RSSI of the signal and hence impact the device's communication throughput. Our second insight is to falsify the above core assumption by \textit{selectively} delaying the direct path beyond reflections and reintroducing ambiguity in AoA measurements. \name can hence preserve all paths to the AP and ensure a consistent high-throughput communication link. 

Yet, selectively applying this delay poses a challenge. For a WiFi signal, which comprises multiple linearly spaced frequency subcarriers, the delay of paths is measured by the additive phase accrued across these subcarriers. Put simply, the phase accrued is proportional to both the amount of delay and the frequency. The individual delays of the direct and reflected paths can hence be estimated via phase measurements across frequencies. A simple way to delay the direct path is to ``pre-code'' additional phases across frequencies to the signal prior to transmission as shown in \cref{fig:intro}(c). However, this also introduces similar delays in the directions of the reflections, allowing the AP to distinguish the direct path AoA as the earliest arriving path. To avoid delaying the reflected paths, we can choose a set of phases across the transmit antennas to direct the signal in the direct path's direction while nulling in the directions of the other reflections, selectively delaying the direct path. To counter the nulling of the reflected paths, we additionally reintroduce the reflections by adding a precoding component to steer power in these directions solely as shown in \cref{fig:intro}(d). This ensures \name's obfuscation closely recreates the original channel, except for the delayed direct path, creating an error in the AoA estimations at the attacking AP. Re-injecting the reflections also preserves the spatial paths, keeping SNR and communication throughput consistent.

With the AoA successfully spoofed by leveraging the reflections in the environment, \name has effectively disabled a core measurement for location estimation. Finally, the precoding applied is non-destructive, unlike other past works~\cite{staat2022irshield, qiao2016phycloak}. This precoding can hence be shared in an encrypted manner to allow a legitimate AP to reverse the effects of the channel obfuscation and conduct localization accurately. \name's obfuscation is tested on commercially available WiFi radios~\cite{warp} and across $xx$ environments in realistic settings. We compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} and mDTrack~\cite{xie2018md}. Through these experiments, we demonstrate the efficiency of \name on WiFi user's location protection. Our experimental results show the localization error degrades by $2.5\times$ and AoA estimation error degrades by $17\times$ at the median after applying \name. 

==> intro/intro-v7.tex <==
% how to locate --> preserve privacy by attacking these ways --> but not broadly applicable --> create software-only by digitally chaging transmission phases --> 
\section{Introduction}

User's location in indoor scenarios is an important aspect of providing a personalized experience. It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automations~\cite{arun2022p2slam}. For these applications and many more, localization accuracy on the order of tens of centimeters is key. Given the widespread presence of WiFi networks indoors, many works~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} have developed systems to provide user location using WiFi signal's physical-layer information. Concerningly, however, many of these systems can operate without the consent of the user. A user connected to just a single access point in an environment can be localized within the required accuracy via the exchange of just a few wireless communication packets~\cite{vasisht2016decimeter}. This compromises user location privacy and opens the door for organizations to potentially commodify~\cite{origin_wireless} this information and spy on users in public spaces~\cite{zhu2018tu} and in homes~\cite{lee2016smart}. This underscores the urgency of safeguarding location privacy from potential intrusions by these localization systems.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/main-intro-fig-crop.pdf}
    \caption{(a) \name-disabled Wi-Fi user can be accurately localized by the Wi-Fi AP thereby introducing the location privacy threat. (b) \name-enabled Wi-Fi user can obfuscate the wireless signals for location privacy protection.}
    \label{fig:main-intro-fig}
\end{figure}

The first line of defense against these intrusive attacks is to anonymize the MAC address with which the user connects to the WiFi network. This masks the user's true identity from the network, and although they can be localized, they cannot be identified. However, recent works~\cite{givehchian2023practical} have shown that chip-level imperfections cause distortions in the signals that can be used to fingerprint devices and identify users despite MAC randomization. As an alternative to masking the user's identity, few works have explored disabling an AP's ability to localize altogether. 
Aegis~\cite{yao2018aegis} deploys a repeater in the environment, tuning the signal's phase and amplitude to prevent a receiver from localizing the user. IRSheild~\cite{staat2022irshield} implements a similar technique but with the use of an Intelligent Reflective Surface to inject phase noise in the WiFi measurements. Although these systems prevent the Angle of Arrival (AoA) determination, they require additional hardware to be deployed in the environments and do not provide a scalable solution for all spaces.
Finally, the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{802.11az} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} demonstrates an attack on 802.11mc FTM, that would still translate to the current systems.
Additionally, WiPeep~\cite{wipeep} proposes a solution to their demonstrated vulnerability in FTM measurements. However, the proposed solution requires changing packet transmission times and is only applicable to future wireless devices.

In light of the limitations of existing works, \name develops a method to protect users of public or enterprise networks from being localized indoors without consent. \name's defense is against the attacker that either could compromise (or add a compromise) one or more of the access points (APs), within these public or enterprise networks. When a user device connects to these networks, they are connected to one of the APs within these networks. 
Single-AP localization solutions have hence been deployed~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi} to tackle these scenarios. 
In most of these applications, three measurements are primarily used to determine a user's location in these scenarios - the signal strength (RSSI), the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. However, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar, ez}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. 

In contrast, a combination of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA can instead be successfully used to localize a user to decimeter-level accuracy and invade their location privacy. 
So, \name's defense model is to ensure degrading the AoA and ToF-based localization accuracy of single-AP localization algorithms to be as inaccurate as RSSI-based localization, i.e., an average of 2-3m accurate location estimation.
Finally, \name makes use of the existing precoding protocols in WiFi~\cite{xie2018md} to precode the signal prior to transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. This approach can be integrated into most existing WiFi devices without the need for additional hardware or firmware changes with minimal disruption to the communication link.

\name's implementation relies on taking advantage of the key underlying principle of most AoA-based localization algorithms.
Accurate AoA estimation forms a core part of estimating the location of the user with decimeter-level accuracy~\cite{spotfi,soltanaghaei2018multipath,arraytrack}. Most multi-antenna access points can measure AoA by observing the relative phase accrued between pairs of their antennas. This relative phase is accrued as the signal travels a slightly larger distance to some antennas than others, as shown in the central inset in \cref{fig:intro}. This physical effect is a consequence of how the signal propagates through the environment and remains consistent regardless of the transmission. Consequently, prior works primarily seek to make changes to the environment by deploying specialized hardware. Does this then preclude a software-only obfuscation scheme? Not necessarily. The measurement of AoA is complicated by the presence of signal reflection(s) in the environment, as shown by the blue arrows in \cref{fig:intro}. Our first insight is to leverage these reflections to create ambiguity in the attacker's AoA estimation by applying a specialized precoding scheme.  


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-usenix-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays only the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to non-zero angle of arrival across receive antennas}
    \label{fig:intro}
\end{figure}


An AP needs to measure the AoA of the direct path signal arriving from the user device to enable localization despite reflections. To distinguish these direct path signals from reflections, existing single-AP solutions~\cite{singleap, chronos, soltanaghaei2018multipath} rely on a core assumption -- the direct path signal travels the least distance and arrives earlier \footnote{delayed by an order of tens of nanoseconds} than the other paths. So, a simple way to provide obfuscation is for a user device to transmit purely in the direction of the reflections, i.e. introduce a null in the direction of the direct path and remove the direct path from the picture as shown in \cref{fig:intro}(b). Despite its effectiveness, this nulling will drastically impact the RSSI of the signal and hence impact the device's communication throughput. Our second insight is to falsify the above core assumption by \textit{selectively} delaying the direct path beyond reflections and reintroducing ambiguity in AoA measurements. \name can hence preserve all paths to the AP and ensure a consistent high-throughput communication link. 

Yet, selectively applying this delay poses a challenge. For a WiFi signal, which comprises multiple linearly spaced frequency subcarriers, the delay of paths is measured by the additive phase accrued across these subcarriers. Put simply, the phase accrued is proportional to both the amount of delay and the frequency. The individual delays of the direct and reflected paths can hence be estimated via phase measurements across frequencies. A simple way to delay the direct path is to ``pre-code'' additional phases across frequencies to the signal prior to transmission as shown in \cref{fig:intro}(c). However, this also introduces similar delays in the directions of the reflections, allowing the AP to distinguish the direct path AoA as the earliest arriving path. To avoid delaying the reflected paths, we can choose a set of phases across the transmit antennas to direct the signal in the direct path's direction while nulling in the directions of the other reflections, selectively delaying the direct path. To counter the nulling of the reflected paths, we additionally reintroduce the reflections by adding a precoding component to steer power in these directions solely as shown in \cref{fig:intro}(d). This ensures \name's obfuscation closely recreates the original channel, except for the delayed direct path, creating an error in the AoA estimations at the attacking AP. Re-injecting the reflections also preserves the spatial paths, keeping SNR and communication throughput consistent.

With the AoA successfully spoofed by leveraging the reflections in the environment, \name has effectively disabled a core measurement for location estimation. This precoding can additionally be shared in an encrypted manner to allow a legitimate AP to reverse the effects of the channel obfuscation and conduct localization accurately. \name's obfuscation is tested on commercially available WiFi radios~\cite{warp}, across 30 locations and over 1000 packets in realistic settings. We compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} and UbiLocate~\cite{pizarro2021accurate}. Through these experiments, we demonstrate the efficiency of \name on WiFi user's location protection. Our experimental results show the localization error degrades by $~2.5\times$ at the median with localization errors as high as $2.8$ m, AoA estimation error degrades by $17\times$ at the median, and ToF estimation error degrades by $~2.5\times$ at the median after applying \name. 

==> intro/intro-v8.tex <==
% how to locate --> preserve privacy by attacking these ways --> but not broadly applicable --> create software-only by digitally chaging transmission phases --> 
\section{Introduction}
{\color{red} ToDo: 1. incorporating the multi-ap scenario. 2. comparing with the carrier-based systems. 3. discuss the privacy implications of meters localization error. 3. DOLOS makes it as bad as RSSI}
User's location in indoor scenarios is an important aspect of providing a personalized experience. It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automations~\cite{arun2022p2slam}. For these applications and many more, localization accuracy on the order of tens of centimeters is key. Given the widespread presence of Wi-Fi networks indoors, many works~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} have developed systems to provide user location using Wi-Fi signal's physical-layer information. Concerningly, however, many of these systems can operate without the consent of the user. A user connected to just a single access point in an environment can be localized within the required accuracy via the exchange of just a few wireless communication packets~\cite{vasisht2016decimeter}. This compromises user location privacy and opens the door for organizations to potentially commodify~\cite{origin_wireless} this information and spy on users in public spaces~\cite{zhu2018tu} and in homes~\cite{lee2016smart}. This underscores the urgency of safeguarding location privacy from potential intrusions by these localization systems.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/main-intro-fig-crop.pdf}
    \caption{(a) \name-disabled Wi-Fi user can be accurately localized by the Wi-Fi AP thereby introducing the location privacy threat. (b) \name-enabled Wi-Fi user can obfuscate the wireless signals for location privacy protection.}
    \label{fig:main-intro-fig}
\end{figure}

The first line of defense against these intrusive attacks is to anonymize the MAC address with which the user connects to the Wi-Fi network. This masks the user's true identity from the network, and although they can be localized, they cannot be identified. However, recent works~\cite{givehchian2023practical} have shown that chip-level imperfections cause distortions in the signals that can be used to fingerprint devices and identify users despite MAC randomization. As an alternative to masking the user's identity, few works have explored disabling an AP's ability to localize altogether. 
Aegis~\cite{yao2018aegis} deploys a repeater in the environment, tuning the signal's phase and amplitude to prevent a receiver from localizing the user. IRSheild~\cite{staat2022irshield} implements a similar technique but with the use of an Intelligent Reflective Surface to inject phase noise in the Wi-Fi measurements. Although these systems prevent the Angle of Arrival (AoA) determination, they require additional hardware to be deployed in the environments and do not provide a scalable solution for all spaces.
Finally, the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{802.11az} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} demonstrates an attack on 802.11mc FTM, that would still translate to the current state-of-the-art wireless sensing systems.
Additionally, WiPeep~\cite{wipeep} proposes a solution to their demonstrated vulnerability in FTM measurements. However, the proposed solution requires changing packet transmission times and is only applicable to future wireless devices.

In light of the limitations of existing works, \name develops a method to protect users from being localized without consent in the public or enterprise networks. \name's defense is against the attacker that either could compromise one or more access points (APs), within the public or enterprise networks. When a user device connects to these networks, they are connected to one of the APs within these networks. 
Single-AP localization solutions have hence been deployed~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi} to tackle these scenarios. So, \name aims to protect user's location privacy against single-AP based attacks in public or enterprise networks. 
\name achieves this location privacy by deteriorating the state-of-the-art  decimeter-accurate localization algorithms~\cite{spotfi,chronos,soltanaghaei2018multipath,arraytrack,ayyalasomayajula2020deep,ma2019wifi} to be only  accurate within a few meters.



Current Single-AP localization algorithms primarily rely on three measurements to determine a user's location in these scenarios - the received signal strength (RSSI), the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. As mentioned, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar, ez}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. 
In contrast, a combination of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA can instead be successfully used to localize a user to decimeter-level accuracy and invade their location privacy. 



So, \name's defense model is to ensure degrading the AoA and ToF-based localization accuracy of single-AP localization algorithms to be as inaccurate as RSSI-based localization, i.e., an average of 2-3m accurate location estimation.
Additionally, \name makes use of the existing precoding protocols in Wi-Fi~\cite{beam_forming_doc} to precode the signal prior to transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. This approach can be integrated into most existing Wi-Fi devices without the need for additional hardware or firmware changes.
Finally, while we ensure user's location privacy we do not want to compromise their connectivity to the Internet and thus \name's design also ensures minimal disruption to the existing communication link.

\name's design principle utilizes the presence of multipath in the environment as its advantages. As shown in Figure~\ref{fig:main-intro-fig}(a), state-of-the-art Single-AP based decimeter-accurate localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az} rely on a simple fact when they use channel state information (CSI) to estimate accurate ToF and AoA -- "direct-path travels the least amount of time in the air". This helps the algorithms to distinguish the direct path parameters from the reflected path's parameters to estimate accurate ToF~\cite{802.11az} and accurate AoA~\cite{spotfi}.
So, \name's key idea is to obfuscate the direct path such that the first of the reflected paths appear to be the shortest travelled path. This would in-turn lead to inaccurate AoA and ToF estimates, degrading their localization accuracy to be of the order of a few meters as shown in Figure~\ref{fig:main-intro-fig}(b).

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-usenix-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays only the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to angle of arrival across receive antennas}
    \label{fig:intro}
\end{figure}

A simple way to make the algorithm estimate the reflected path to be shortest path is to simply remove the direct path as shown in Figure~\ref{fig:intro}(b). Unfortunately, this removes one of the dominant path for connectivity, reducing the throughput for the user connection. Thus we cannot simply remove the direct path signal.
Another key observation we note here is that, for a given location of the user and the Wi-Fi AP, we cannot change the directions or AoAs of the received signal as that depends on the geometry of the environment that is out of our control or would need additional hardware deployments that compromises deployability of \name's design. So, in \name we identify that the only way we can let the receiver perceive the reflected path to be the shortest travelled path is if we can "delay" the signal along the direct-path direction.

Since the multiple reflections (multipath) in the environment, including the direct path and the reflected paths, have a common source, a naive delay applied to the transmitted signal unfortunately would delay all the signals in all directions by the same amount as shown in Figure~\ref{fig:intro}(c). This would not lead to the intended effect of ``selective-delay" of just the direct-path that is shown in Figure~\ref{fig:intro}(d). Here \name makes a key observation that most of the modern user device relies on MIMO communication and thus have multiple antennas for transmission. This would imply that the user device can beamform~\cite{beam_forming_doc} the signal independently in each of the signal departure directions or angle-of-departures (AoD). Thus, in \name we design a precoding matrix that beamforms the transmitted signal while ensuring that both:
(a) The beamforming along the direct path with additional delay is orthogonal to the reflected path's transmitted directions.
(b) The beamforming performed for the reflected paths without additional delays is orthogonal to the newly delayed reflected path's transmitted directions.
We then apply the sum of these two nearly orthogonal beams to the transmitted signal to achieve the perceived affect of selective delay of the direct path signal, thus successfully obfuscating the direct path signal with a reflected path signal. Which will ensure incorrect AoA and ToF estimation for the state-of-the-art localization algorithms, increasing their errors from decimeters to a few meters.

\name's obfuscation is tested on commercially available Wi-Fi radios~\cite{warp}, across 30 locations and over 1000 packets in realistic settings. \name's design degrades the accuracy for fundamental predictions of AoA and ToF that are used by the state-of-the-art Single-AP localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az}. So we compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} (relies fundamentally on AoA) and UbiLocate~\cite{pizarro2021accurate} (relies fundamentally on ToF). Through these experiments, we demonstrate the efficiency of \name on Wi-Fi user's location protection. Our experimental results show the localization error degrades by $~2.5\times$ at the median with localization errors as high as $2.8$ m, AoA estimation error degrades by $17\times$ at the median, and ToF estimation error degrades by $~2.5\times$ at the median after \name. 

==> intro/intro-v9.tex <==
% how to locate --> preserve privacy by attacking these ways --> but not broadly applicable --> create software-only by digitally chaging transmission phases --> 
\section{Introduction}
% {\color{red} ToDo: 1. incorporating the multi-ap scenario. 2. comparing with the carrier-based systems. 3. discuss the privacy implications of meters localization error. 3. DOLOS makes it as bad as RSSI}

User's location in indoor scenarios is an important aspect of providing a personalized experience.
It provides context to a user's activity~\cite{ayyalasomayajula2020deep}, aids in navigation and wayfinding~\cite{ayyalasomayajula2020locap}, and paves the way for smart building automations~\cite{arun2022p2slam}.
For these applications and many more, localization accuracy on the order of tens of centimeters is key.
This led to accurate Wi-Fi based indoor localization research for more than two-decades that started with signal strength (RSSI) localization systems that can provide only a meter-accurate localization~\cite{radar,zee} to many systems~\cite{spotfi, ayyalasomayajula2020deep, wipeep, vasisht2016decimeter,luo2023meta2locate} that provide tens of centimeters-accurate user location using Wi-Fi signal's physical-layer information. 
Concerningly, many of these systems can operate without the consent of the user. 
% A user connected to just a single access point in an environment can be localized within the required accuracy via the exchange of just a few wireless communication packets~\cite{vasisht2016decimeter}. 
This compromises user location privacy and opens the door for organizations to potentially commodify~\cite{origin_wireless} this information and spy on users in public spaces~\cite{zhu2018tu} and in homes~\cite{lee2016smart}.
This underscores the urgency of safeguarding location privacy from potential intrusions by these localization systems.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/main-intro-fig-crop.pdf}
    \caption{(a) \name-disabled Wi-Fi user can be accurately localized by the Wi-Fi AP thereby introducing the location privacy threat. (b) \name-enabled Wi-Fi user can obfuscate the wireless signals for location privacy protection.}
    \label{fig:main-intro-fig}
\end{figure}

Current Wi-Fi based localization algorithms primarily rely on three measurements to determine a user's location in these scenarios - the received signal strength (RSSI), the time of flight (ToF) of the signal, and the angle of arrival (AoA) of the signal. As mentioned, RSSI-based systems commonly provide accuracy in the order of meters~\cite{radar, ez}, meaning users can be localized in different rooms or even different floors. This level of accuracy does not pose a threat to a user's privacy. 
In contrast, a mixture of ToF (802.11mc, 802.11az~\cite{802.11az}) and AoA  measurements can be successfully used to localize a user to decimeter-level accuracy and invade their location privacy. 

The first line of defense against these intrusive attacks is to anonymize the MAC address with which the user connects to the Wi-Fi network. This masks the user's true identity from the network, and although they can be localized, they cannot be identified. However, recent works~\cite{givehchian2023practical} have shown that chip-level imperfections cause distortions in the signals that can be used to fingerprint devices and identify users despite MAC randomization. 
An alternative to masking user identity is to disrupt the localization measurements.
the latest Fine-Grained Positioning (FGP, 802.11az)~\cite{802.11az} proposes a more secure FTM measurement; however, the attack model in WiPeep~\cite{wipeep} demonstrates an attack on 802.11mc FTM, that would still translate to the current state-of-the-art wireless sensing systems.
Additionally, WiPeep~\cite{wipeep} proposes a solution to their demonstrated vulnerability in FTM measurements. However, the proposed solution requires changing packet transmission times and is only applicable to future wireless devices.
A few works have explored disabling an AP's ability to localize altogether, by deploys a repeater~\cite{yao2018aegis} or Smart surface~\cite{staat2022irshield} in the environment, tuning the signal's phase and amplitude to prevent a receiver from localizing the user. Although these systems prevent the Angle of Arrival (AoA) determination, they require additional hardware to be deployed in the environments and do not provide a scalable solution for all spaces.


In light of the limitations of existing works, \name develops a method to protect users from being localized without consent in the public or enterprise networks. \name's defense is against the attacker that either could compromise one or more access points (APs), within the public or enterprise networks. When a user device connects to these networks, they are connected to one of the APs within these networks. 
\name achieves this location privacy by deteriorating the state-of-the-art decimeter-accurate localization algorithms~\cite{spotfi,chronos,soltanaghaei2018multipath,arraytrack,ayyalasomayajula2020deep,ma2019wifi} to be only as accurate as a few meters or the RSSI-based localization systems~\cite{radar,zee}, back-tracking decades of research in improving Wi-Fi based Indoor Localization. For example, for indoor scenarios where user needs to be located accurate to be within their cubicle in the office or an aisle in a shopping complex would be mislocated to an incorrect cubicle or aisle.



\begin{comment}
    Wi-Fi based localization has been recongozed and imprtatn for decimeter accurate lcoation.
    Ther research started at a few meters accurate to now being decimeter acccurate, but does not have user consent. 

    Rssi based meter level accurate systems have been improved by the current works achieve decimeter accurate by doing aoa, tof and do not require consent, hence privacy concerns.

    Some works for privacy falls short of doing a good job.

    We do a good job by making the decimeter systems as inaccurate as rssi-systems or accurate to only a few meters. Our system is also protocol-compliant and communication preserving. So let us understand what makes this challenging.

    First challenge is that the APs have multiple antennas that can resolve multiple paths through aoa estimation, and identify the direct path using the notion that it is the least travelled and most consistent path.

    A dumb way to do this is nulling but reduces the communication link, so we firstly precode such that the ap does not perceive the correct direct path and also does not remove any paths thus maintatining communication link.

    The second challenge, is that delaying one-path creates delays or ghost peaks across all the paths like done in mirage, so we need to ensure that the direct path and multipath precoding matrices are orthogonal and that we add delay to only the direct path's precoding vector.

    Finally, we address a few real world problems of consistency of the durect path and multiple collaborative APs, by adding random delays and obfuscating one AP at a time across all the environment AP respectively.

    We tested, and got awesome results.    
\end{comment}

So, \name's defense model is to ensure degrading the AoA and ToF-based localization accuracy of the Wi-Fi localization algorithms to be as inaccurate as RSSI-based localization, i.e., an average of 2-3m median accurate location estimation.
Additionally, \name makes use of the existing precoding protocols in Wi-Fi~\cite{beam_forming_doc} to precode the signal prior to transmission at a software level to obfuscate the AoA measurement and build a broadly applicable solution. 
This allows \name to readily integrate into most existing Wi-Fi devices and provide user-location privacy without the need for additional hardware or firmware changes.
Finally, to ensure user's location privacy without compromising their connectivity to the Internet, we design \name to have minimal disruption to the existing communication link.

\name's design principle takes advantage of the multipath characteristics of indoor environments that has driven the research in MIMO communication~\cite{wallace2002modeling} and sensing~\cite{soltanaghaei2018multipath,kotaru2017position}.
As shown in Figure~\ref{fig:main-intro-fig}(a), state-of-the-art Single-AP based decimeter-accurate localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az} rely on a simple fact when they use channel state information (CSI) to estimate accurate ToF and AoA -- "direct-path travels the least amount of time in the air". This helps the algorithms to distinguish the direct path parameters from the reflected path's parameters to estimate accurate ToF~\cite{802.11az} and accurate AoA~\cite{spotfi}.
So, \name's key idea is to obfuscate the direct path such that the first of the reflected paths appear to be the shortest travelled path. This would in-turn lead to inaccurate AoA and ToF estimates, degrading their localization accuracy to be of the order of a few meters as shown in Figure~\ref{fig:main-intro-fig}(b).

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/intro-fig-usenix-crop.pdf}
    \caption{(a) Direct path (green) arrives earlier at the AP due to shorter path length (b) Nulling the direct path obfuscates the AoA, but reduces signal strength (c) Naively delaying the paths does not change the relative arrival times, (d) \name selectively delays only the direct path, breaking the assumption in (a). Inset: relative phase accrued from path length difference due to angle of arrival across receive antennas}
    \label{fig:intro}
\end{figure}

A simple way to make the algorithm estimate the reflected path to be shortest path is to simply remove the direct path as shown in Figure~\ref{fig:intro}(b). Unfortunately, this removes one of the dominant path for connectivity, reducing the throughput for the user connection. Thus we cannot simply remove the direct path signal.
Another key observation we note here is that, for a given location of the user and the Wi-Fi AP, we cannot change the directions or AoAs of the received signal as that depends on the geometry of the environment that is out of our control or would need additional hardware deployments that compromises deployability of \name's design. So, in \name we identify that the only way we can let the receiver perceive the reflected path to be the shortest travelled path is if we can "delay" the signal along the direct-path direction.

Since the multiple reflections (multipath) in the environment, including the direct path and the reflected paths, have a common source, a naive delay applied to the transmitted signal unfortunately would delay all the signals in all directions by the same amount as shown in Figure~\ref{fig:intro}(c). This would not lead to the intended effect of ``selective-delay" of just the direct-path that is shown in Figure~\ref{fig:intro}(d). Here \name makes a key observation that most of the modern user device relies on MIMO communication and thus have multiple antennas for transmission. This would imply that the user device can beamform~\cite{beam_forming_doc} the signal independently in each of the signal departure directions or angle-of-departures (AoD). Thus, in \name we design a precoding matrix that beamforms the transmitted signal while ensuring that both:
(a) The beamforming along the direct path with additional delay is orthogonal to the reflected path's transmitted directions.
(b) The beamforming performed for the reflected paths without additional delays is orthogonal to the newly delayed reflected path's transmitted directions.
We then apply the sum of these two nearly orthogonal beams to the transmitted signal to achieve the perceived affect of selective delay of the direct path signal, thus successfully obfuscating the direct path signal with a reflected path signal. Which will ensure incorrect AoA and ToF estimation for the state-of-the-art localization algorithms, increasing their errors from decimeters to a few meters.

\name's obfuscation is tested on commercially available Wi-Fi radios~\cite{warp}, across 30 locations and over 1000 packets in realistic settings. \name's design degrades the accuracy for fundamental predictions of AoA and ToF that are used by the state-of-the-art Single-AP localization algorithms~\cite{vasisht2016decimeter, soltanaghaei2018multipath,liu2021rfloc,shoudha2023wifi,ma2019wifi,802.11az}. So we compare the accuracy degradation provided by \name when using two state-of-the-art localization systems -- SpotFi~\cite{spotfi} (relies fundamentally on AoA) and UbiLocate~\cite{pizarro2021accurate} (relies fundamentally on ToF). Through these experiments, we demonstrate the efficiency of \name on Wi-Fi user's location protection. Our experimental results show the localization error degrades by $~YY\times$ at the median with localization errors as high as $ZZ$ m, AoA estimation error degrades by $XX\times$ at the median, and ToF estimation error degrades by $~XX\times$ at the median after \name. 

==> results/results-v2.tex <==
% !TEX root = paper.tex
\section{Implementation}\label{sec:imp}

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/ap_user_warps.pdf}
%    \caption{The left two figures show the Wi-Fi AP and user respectively and the rightmost figure shows the experiment setup, where the red triangle indicates the static Wi-Fi AP's position and the blue dot shows the Wi-Fi user's possible position in the typical office room.}
%    \label{fig:ap:warps}
%\end{figure}

In this section, we briefly go over the hardware system setup that involves the static (infrastructure) Wi-Fi AP, and the movable Wi-Fi user on which the DOLOS algorithm would be deployed.
%\begin{figure*}
%\centering
%    \begin{minipage}{0.24\linewidth}
%        \includegraphics[width=\linewidth]{figures/loc_cdf-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \begin{minipage}{0.24\linewidth}
%        \includegraphics[width=\linewidth]{figures/aoa_cdf-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \begin{minipage}{0.24\linewidth}
%        \includegraphics[width=\linewidth]{figures/rssi_cdf-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \begin{minipage}{0.24\linewidth}
%        \includegraphics[width=\linewidth]{figures/ghosts-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \caption{\textbf{End-to-End Evaluation for \name:} (a) Shows the CDF of the final user localization error in meters using the AoA estimated from SpotFi and the range from the FTM measurements. (b) Shows the CDF of the final AoA error in degrees using the AoA estimated from SpotFi. (c) Shows the CDF of the RSSI in dBm. (d) Shows the CDF of the ambiguity measure  for \name, no obfuscation, \name's CDB as BF only, and \name's CDB+N as BF+ NULL }
%    \label{fig:end-to-end}
%\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/mirage_exp.pdf}
    \caption{\todo{fix fig} Experimental Setup: On the left is the Dual-WARP setup that we use as the attacking AP, the rightmost image shows the User WARP device that is mounted on a robot that collects ground-truth location for the user device. The blue dots are the user locations \name is tested at, and the AP is at origin (0,0). }
    \label{fig:ap:warps}
\end{figure}

\noindent \textbf{Wi-Fi AP.} We use a software-defined radio (WARP~\cite{warp}) as the Wi-Fi AP instrumented with four antennas working at the 5Ghz Wi-Fi band as shown in Fig.~\ref{fig:ap:warps}. This Wi-Fi AP will mainly leverage the SpotFi algorithm to create the AoA-ToF profile, which can be used to localize the Wi-Fi user accurately. This Wi-Fi AP will connect to the central controller (i.e. laptop) for data processing and applying the super-resolution indoor localization algorithm (SpotFi). This WARP-based Wi-Fi AP is co-located with an ASUS AP~\cite{asus} that can be used to obtain the ToF of packets exchanged between the Wi-Fi AP and user. As such, the Wi-Fi AP can leverage the derived AoA and ToF to localize the Wi-Fi user. 




\noindent \textbf{Wi-Fi User.} We still use a software-defined radio (WARP) as the Wi-Fi user as shown in  Fig.~\ref{fig:ap:warps}. Specifically, we synchronize two WARPs as one Wi-Fi user instrumented with four antennas. Since the Wi-Fi user can move around in the indoor environment, we deploy our radios on a robot to emulate the Wi-Fi user's movement.  The Wi-Fi user is still connected to the central controller (in this case, a laptop ) for applying the \name to obfuscate the Wi-Fi user's location. We also assume there is an ASUS AP co-located with the Wi-Fi user that can exchange packets with the ASUS AP co-located with the Wi-Fi AP for ToF estimation. 


\noindent \textbf{Experimental Setup.} The Wi-Fi AP and user will connect to a central controller, which can perform the obfuscation and channel estimation for localization. To measure the performance of our system, we conduct experiments in the indoor area (i.e. an office building). Specifically, the Wi-Fi user colocated with an ASUS AP can move around in the indoor environment on an emulated robot as shown in Fig.~\ref{fig:ap:warps}, and the Wi-Fi AP co-located with an ASUS AP is static in the indoor environment.  Wi-Fi AP and user can communicate with each other over the 5GHz WiFi spectrum, while a pair of ASUS APs can communicate with each other in another frequency band for ToF estimation. During the communication, the Wi-Fi AP may localize the Wi-Fi user with the estimated AoA from WARPs and ToF from ASUS APs, which will introduce the location privacy threat. So, the Wi-Fi user can apply our \name algorithm to protect his or her location privacy by obfuscating the direct-path signals seen at the Wi-Fi AP.

\begin{figure*}
\begin{subfigure}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{results/figures/localization_error.pdf}
\caption{}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{results/figures/aoa_error.pdf}
\caption{}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\centering
\includegraphics[width=\textwidth]{results/figures/ftm_error.pdf}
\caption{}
\end{subfigure}
\caption{(a) Showcases end-end localization error. (b) Showcases AoA estimation error by SpotFi with \name's obfuscation turned on and off. (c) Showcases the FTM error from Ubilocate~\cite{pizarro2021accurate} \todo{add tof+dolos}}
\label{fig:end-to-end}
\end{figure*}

\section{Evaluation}\label{sec:results}

%The best way to measure the effectiveness of our algorithm, we have assumed accurate range estimates as would be provided by Wi-Peep\cite{wipeep} to perform end-to-end localization of the user device. We perform this analysis under various assumptions to test the robustness of \name.



To evaluate the efficiency of \name, our evaluation consists of microbenchmarks and end-to-end system-level tests. We first report the robustness of our location obfuscation approach and system in the dynamic indoor environment. Then, we show the effect of location obfuscation on the wireless communication performance. At last, We evaluate the localization accuracy with and without \name to demonstrate the end-to-end location obfuscation errors in the dynamic indoor environment. Specifically, we will show the localization errors, AoA estimation errors, and ToF estimation errors.    

%The localization accuracy without \name, then the localization accuracy with \name's beamforming only, and \name's implementation with beam-forming and nulling. We also demonstrate the effect of user motion on \name, and robustness of \name towards using approximate downlink CSI for obfuscation.

%We have also measured the ratio number of peaks in the 2D SpotFi profile with and without obfuscation, that we call ambiguity measure$\mathcal{A}$, where if there are $N_{wo}$ and $N_w$ peaks correspondingly for without and with obfuscation, i.e. $\mathcal{A} = N_{wo}/N_w$, where ideal value is 1, and slightly $>1$ and any value $<1$ indicates false and ghost peaks occurring. 

%We also report the RSSI degradation, where we measure the RSSI of the measurement with and without obfuscation at each location $RSSI_{deg} (dB) = RSSI_{wo} (dB) - RSSI_w (dB)$.

% \todo{do we need microbenchmark going over the when $v_d$ will suffice and when $n_r$ is needed?}

\subsection{End-to-end Localization Errors}

\todo{Add md-track aoa results as well}

\subsubsection{Localization Errors}
The localization error is defined as the difference between the estimated location and the ground-truth location of the Wi-Fi user.

\noindent \textbf{Method.} To show the localization errors of \name, we conduct experiments in an office building. The Wi-Fi user's location is estimated through the uplink obfuscated channels at the Wi-Fi AP through the super-resolution algorithm (e.g., SpotFi).

\noindent \textbf{Results.} Fig.~\ref{fig:end-to-end}(a) shows the CDF of the localization error while using state-of-the-art localization, by estimating ToF with Ubilocate~\cite{pizarro2021accurate} and AoA using SpotFi~\cite{spotfi}. We then apply \name's obfuscation to the AoA prediction. We also observe that the minute delays applied by \name does not affect the errors in ToF. As we can see, the median localization error is around 0.8 m. This fine-grained accuracy can easily pinpoint a user in a specific room in an office, aisle at a grocery store or a kiosk at a mall, robbing the user of their privacy in these public spaces.  However, with \name activated, the localization error increases {$2.5\times$}, with the median localization error is around 1.86 m. This implies, with \name's obfuscation enabled, even state-of-art localization systems' accuracy reduces to that of RSSI based systems and indicating the significance of \name algorithm to obfuscate the Wi-Fi user's location. 

\subsubsection{AoA Errors}
Since \name attempts to obfuscate the angle-of-arrival information of the Wi-Fi user, it's crucial to demonstrate the performance of \name on AoA obfuscation. To do so, we plan to show the AoA errors after applying our \name algorithm. 

\noindent \textbf{Method.} To localize the Wi-Fi user, the Wi-Fi AP usually leverages the direct-path AoA and ToF for Wi-Fi user localization. Here, we report the AoA estimation error at the Wi-Fi AP with, and without obfuscation. The AoA estimation error is defined as the difference between the ground-truth AoA and the estimated AoA with a super-resolution localization algorithm (SpotFi). 


\noindent \textbf{Result.} Fig.~\ref{fig:end-to-end}(b) shows the CDF of the AoA errors while using SpotFi without obfuscating the channel and with \name's obfuscation activated. As we can see, the median  and $90^\mathrm{th}$ percentile AoA error without \name is around 2.3 and 7.8 degrees respectively. However, this AoA predictions with SpotFi severely degrades by $17\times$ at median and $6\times$ at the $90^\mathrm{th}$ percentile once \name obfuscates the channel. This is because \name can obfuscate the direct-path AoA and confuse the Wi-Fi AP to use the random multipath for Wi-Fi user localization, resulting in high AoA estimation errors. 
% \subsubsection{ToF Errors}
% \subsubsection{Success Rate of Location Obfuscation}
% \subsubsection{Location Obfuscation Time}

\subsection{Microbenchmarks}

% \subsubsection{Effect of Direct Path Beamforming}
% \subsubsection{Effect of Delaying}


\begin{figure*}
    \begin{subfigure}{0.33\linewidth}
        % \includegraphics[width=\linewidth]{results/figures/aoa_error_past_present.pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}
        \includegraphics[width=\linewidth]{results/figures/loc_error_past_present.pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}
        \includegraphics[width=\linewidth]{results/figures/aoa_error_past_present.pdf}
        \caption{}
    \end{subfigure}
    \caption{\todo{Add throughput plot here}}
    \label{fig:enter-label}
\end{figure*}

\subsubsection{Testing Robustness under motion}

To measure the robustness of \name under motion. We do the experiments by leveraging the downlink channels that are measured when the Wi-Fi user is moving. These measured downlink channels will be used by the Wi-Fi user to obfuscate the Wi-Fi AP, such that he/she cannot accurately identify the direct-path AoA for localization. To do so, the Wi-Fi user will use the downlink channels from the previous time step. Between these time-steps, the user has moved an average of ~$7$ cm. \cref{fig:end-to-end}(a) showcases the localization error when using this stale precoding vector. As we can see, the median localization error is around 1.7m and 90th percentile localization error is around 2.9m, which are not significantly degraded in comparison to using the current precoding vector. Similarly, \cref{fig:end-to-end}(b) shows the AoA estimation error when using this stale precoding vector for location obfuscation. As we can see, the median AoA estimation error is around 36.71 degree and the 90th percentile AoA estimation error is around 50 degree, which is closed to using the current precoding vector for location obfuscation. This is because the wireless channel is quasi-staic and our location obfuscation approach is resilient to the dynamic wireless environmet.

%1.7 m error median, 2.9 m 90th percentile 
%36.71 deg error median, 50 deg 90th percentile. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{results/figures/mb-comp-need-crop.pdf}
    \caption{\todo{fix figure and caption} (a) Original channel (b) Channel without compensation (c) channel with compensation}
    \label{fig:enter-label}
\end{figure}

\begin{figure*}
    \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{results/figures/avg_need.pdf}    
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{results/figures/p_inj_need.pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{results/figures/mp_diversity.pdf}
        \caption{}
    \end{subfigure}
    \caption{\todo{add averaging cdf's here}}
    \label{fig:enter-label}
\end{figure*}

\subsubsection{Need for compensating direct path precoder} 

In \cref{sec:design-bf} we discussed the need to apply additional compensation $\frac{1}{\alpha}\exp(-\iota \phi)$ to the direct path precoder. We found this necessary as the beamformer which null in the directions of reflections may not completely align with the direction of the direct path. In \cref{fig:enter-label}, we showcase the importance of this compensation parameter. We find that without the explicit phase correction applied across the frequency subcarriers, there are mulitple expressions for the time of flight of the direct path signal. This creates a smearing effect in the AoA-ToF profile and lead to the discovery that the channel is being obfuscated.  

\subsubsection{FTM measurement accuracy}

We measure the time of flight of the signal using FTM~\cite{pizarro2021accurate}. For each location we conduct FTM for a period of 2 seconds and transmit ~1000 packets to improve averaging gain and accuracy. Due to hardware offset, we observe a constant bias which is calibrated for prior to the experiment. \cref{fig:end-to-end}(c) showcases the FTM accuracy post calibration, providing a median and $90^\mathrm{th}$ percentile ranging accuracy of 0.3 m and 0.65 m.   

% \subsubsection{Effect of \name on Wireless Communication Performance}


%\subsubsection{RSSI Performance}
%It is important to maintain the wireless communication throughput while protecting the Wi-Fi user's location privacy. This requires our \name to not degrade the network throughput. 

%\noindent \textbf{Method.} To demonstrate this, we report the RSSI at the Wi-Fi AP, which can indicate the network performance of our system. We expect the RSSI estimated at the Wi-Fi AP should not be significantly degraded to maintain good wireless communication performance even after obfuscating the Wi-Fi user's location. 


%\noindent \textbf{Result.} Fig.~\ref{fig:end-to-end}(c) shows the CDF of RSSI without \name, with beamforming and delaying, with beamforming-nulling and delaying. As we can see, the RSSI is quite similar with or without obfuscation, which is around -76dBm. Even though \name obfuscates the direct-path signals, the wireless communication link is not significantly affected. This is because the wireless communication signals is going through the multipath environment, which can explore the multiplexing gain introduced by the space diversity. 

%\subsubsection{Ambiguity Tolerance} 
%The design of \name could introduce some ghost peaks in the multipath profile, which may affect our obfuscation performance. This is because \name tries to obfuscate the Wi-Fi AP's localization algorithm such that it cannot accurately identify the direct-path signals. 

%\noindent \textbf{Method.} To do so, we demonstrate the ambiguity tolerance of \name using the ambiguity measure, which indicates how many ghost peaks have been introduced by our obfuscation algorithm. We should expect that the ambiguity measure is larger than one when our obfuscation algorithm does not introduce extra ghost peaks in the multipath profile. 

%\noindent \textbf{Result.} Fig.~\ref{fig:end-to-end}(d) shows the CDF of the ambiguity measure with beamforming and delaying and beamforming-nulling and delaying. As we can see, the median ambiguity measure is around 1.2, which indicates that our obfuscation algorithms do not introduce new ghost peaks. As a result, our obfuscation algorithms can accurately obfuscate the Wi-Fi AP, which will not be able to localize the Wi-Fi user accurately through the super-resolution localization algorithm. 


%\begin{figure*}
%\centering
%    \begin{minipage}{0.3\linewidth}
%        \includegraphics[width=\linewidth]{figures/ambiguity_motion-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \begin{minipage}{0.3\linewidth}
%        \includegraphics[width=\linewidth]{figures/rssi_motion-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \begin{minipage}{0.3\linewidth}
%        \includegraphics[width=\linewidth]{figures/loc_motion-crop.pdf}
%        \subcaption{}
%    \end{minipage}
%    \caption{\textbf{Robusntess under Motion for \name:} Shows the results when the \name's downlink channel measurement is $d$m away from the actual user location, which would be the case under user's motion (a) The CDF of the ambiguity measure of \name for $d={0m,0.1m,0.2m,0.5m}$ (b) CDF of RSSI degradation of \name for $d={0m,0.1m,0.2m,0.5m}$
%    (c) CDF of the final user localization error in meters for $d={0m,0.1m,0.2m,0.5m}$. Showing that \name can tolerate old downlink channels from as far as $<50$~cm without degradation in the performance.}
%    \label{fig:end-to-end:motion}
%\end{figure*}  






% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/ghosts.pdf}
%     \caption{.}
%     \label{fig:ghosts}
% \end{figure}






